Compressed Skinning for Facial Blendshapes

We present a new method to bake classical facial animation blendshapes into a fast linear blend skinning representation. Previous work explored skinning decomposition methods that approximate general animated meshes using a dense set of bone transformations; these optimizers typically alternate between optimizing for the bone transformations and the skinning weights.We depart from this alternating scheme and propose a new approach based on proximal algorithms, which effectively means adding a projection step to the popular Adam optimizer. This approach is very flexible and allows us to quickly experiment with various additional constraints and/or loss functions. Specifically, we depart from the classical skinning paradigms and restrict the transformation coefficients to contain only about 10% non-zeros, while achieving similar accuracy and visual quality as the state-of-the-art. The sparse storage enables our method to deliver significant savings in terms of both memory and run-time speed. We include a compact implementation of our new skinning decomposition method in PyTorch, which is easy to experiment with and modify to related problems.

==> Backups.tex <==
When precise measurements are needed, prior work relies on either 1) reflective markers attached to a motion capture suit or glued to the skin \cite{park2006capturing}, or 2) painting colored patterns on the skin \cite{bogo2017dynamic}.

Those are the strong points that I want to put in the introduction:
\begin{itemize}
    \item Uniquely label the markers, only relying on local features, which allows us to capture more challenging poses.
    \item Directly get 4D data without relying on temporal tracking, human body shape or kinematics model
    \item Can be directly used as ground truth data
    \item Robust despite large deformations of human skin and self-occlusion
    \item Allow parallel processing
    \item Rely on standard RGB or monochrome sensors
    \item passive light only
\end{itemize}

This is how I plan to fulfill the rest of the Introduction:

\paragraph{Part 1,} downsides of two ways to get accurate measurements (reflective markers, painting colored patterns)
\begin{itemize}
    \item \textbf{Problem of reflective markers}: marker labeling is hard, which limits the total number of markers that can be used.
    \item \textbf{Problem of painting colored patterns}: relies on the texture, which have to be generated from the geometric registration. Limited volume of capture. All those limited the variety of poses that can be captured. Besides, the price of the system is prohibitive.
\end{itemize}

\paragraph{Part 2}Our solution:
\begin{itemize}
    \item Our solution is, putting fiducial markers on the subject's body, using a special capture suit.
    \item Unlike painting colored patterns directly on skin, the suit allows us to print a sophisticatedly designed high-resolution image on it, which includes more than one thousand fiducial markers enabling both accurate localization, and inference of unique labels which is temporally invariant for each marker. The suit naturally moves along with the body, thus the markers represent temporally consistent locations on the body.
    \item The  localization and labelling of fiducial markers, which is just a small patch on the suit, only relies on the local suit feature, thus is robust despite large deformations of human skin and self-occlusion.
    \item Consequently, we are able to capture a more variety of motions, including challenging motions, like yoga poses with significant self occlusions, and like rolling on the ground which requires large capture volume.
    \item By reconstructing those markers, we directly obtain the 4D data of human motion with a unique label for each marker, without requiring registration of template mesh, prior human body shape or kinematics model. Instead, our trajectories can be used as ground truth data.
    \item The independence between frames, also allows us to process them in parallel.
    \item Low cost of only relying on standard RGB or monochrome sensors 
\end{itemize}

Then I will talk about our evaluation method and discuss our results.
